Interactive Elicitation of Knowledge on Feature Relevance Improves Predictions in Small Data Sets

Providing accurate predictions is challenging for machine learning algorithms when the number of features is larger than the number of samples in the data. Prior knowledge can improve machine learning models by indicating relevant variables and parameter values. Yet, this prior knowledge is often tacit and only available from domain experts. We present a novel approach that uses interactive visualization to elicit the tacit prior knowledge and uses it to improve the accuracy of prediction models. The main component of our approach is a user model that models the domain expert's knowledge of the relevance of different features for a prediction task. In particular, based on the expert's earlier input, the user model guides the selection of the features on which to elicit user's knowledge next. The results of a controlled user study show that the user model significantly improves prior knowledge elicitation and prediction accuracy, when predicting the relative citation counts of scientific documents in a specific domain.

==> references <==
@article{afrabandpey2016interactive,
  title={Interactive Prior Elicitation of Feature Similarities for Small Sample Size Prediction},
  author={Afrabandpey, Homayun and Peltola, Tomi and Kaski, Samuel},
  journal={arXiv preprint arXiv:1612.02802},
  year={2016}
}

@article{alsallakh2014visual,
  title={Visual methods for analyzing probabilistic classification data},
  author={Alsallakh, Bilal and Hanbury, Allan and Hauser, Helwig and Miksch, Silvia and Rauber, Andreas},
  journal={IEEE Transactions on Visualization and Computer Graphics},
  volume={20},
  number={12},
  pages={1703--1712},
  year={2014},
  publisher={IEEE}
}


@inproceedings{bird2006nltk,
  title={{NLTK: the natural language toolkit}},
  author={Bird, Steven},
  booktitle={Proc of the COLING/ACL on Interactive presentation sessions},
  pages={69--72},
  year={2006}
}

@inproceedings{brooks2015featureinsight,
  title={{FeatureInsight: Visual support for error-driven feature ideation in text classification}},
  author={Brooks, Michael and Amershi, Saleema and Lee, Bongshin and Drucker, Steven M and Kapoor, Ashish and Simard, Patrice},
  booktitle={Proc of IEEE VAST},
  pages={105--112},
  year={2015}
}
  

@article{costello2014community,
  title={{A community effort to assess and improve drug sensitivity prediction algorithms}},
  author={Costello, James C and Heiser, Laura M and Georgii, Elisabeth and G{\"o}nen, Mehmet and Menden, Michael P and Wang, Nicholas J and Bansal, Mukesh and Hintsanen, Petteri and Khan, Suleiman A and Mpindi, John-Patrick and others},
  journal={Nature Biotechnology},
  volume={32},
  number={12},
  pages={1202--1212},
  year={2014},
  publisher={Nature Publishing Group}
}

@article{daee2016knowledge,
  title={Knowledge Elicitation via Sequential Probabilistic Inference for High-Dimensional Prediction},
  author={Daee, Pedram and Peltola, Tomi and Soare, Marta, and Kaski, Samuel},
  journal={arXiv preprint arXiv:1612.03328},
  year={2016}
}


@article{el2009kp,
  title={{KP-Miner: A keyphrase extraction system for English and Arabic documents}},
  author={El-Beltagy, Samhaa R and Rafea, Ahmed},
  journal={Information Systems},
  volume={34},
  number={1},
  pages={132--144},
  year={2009},
  publisher={Elsevier}
}

@book{friedman2001elements,
  title={{The elements of statistical learning}},
  author={Friedman, Jerome and Hastie, Trevor and Tibshirani, Robert},
  volume={1},
  year={2001},
  publisher={Springer, Berlin: Springer Series in Statistics}
}


@article{genkin2007large,
  title={{Large-scale Bayesian logistic regression for text categorization}},
  author={Genkin, Alexander and Lewis, David D and Madigan, David},
  journal={Technometrics},
  volume={49},
  number={3},
  pages={291--304},
  year={2007},
  publisher={Taylor \& Francis}
}


@article{hoerl1970ridge,
  title={{Ridge regression: Biased estimation for nonorthogonal problems}},
  author={Hoerl, Arthur E and Kennard, Robert W},
  journal={Technometrics},
  volume={12},
  number={1},
  pages={55--67},
  year={1970},
  publisher={Taylor \& Francis Group}
}

@inproceedings{kapoor2010interactive,
  title={Interactive optimization for steering machine classification},
  author={Kapoor, Ashish and Lee, Bongshin and Tan, Desney and Horvitz, Eric},
  booktitle={Proc of the SIGCHI Conference on Human Factors in Computing Systems},
  pages={1343--1352},
  year={2010},
  organization={ACM}
}

@inproceedings{kogan2009predicting,
  title={{Predicting risk from financial reports with regression}},
  author={Kogan, Shimon and Levin, Dimitry and Routledge, Bryan R and Sagi, Jacob S and Smith, Noah A},
  booktitle={Proc of NAACL HLT},
  pages={272--280},
  year={2009}
}

@inproceedings{lewis1992feature,
  title={{Feature selection and feature extraction for text categorization}},
  author={Lewis, David D},
  booktitle={Proc of the Workshop on Speech and Natural Language},
  pages={212--217},
  year={1992}
}

@inproceedings{may2011guiding,
  title={Guiding feature subset selection with an interactive visualization},
  author={May, Thorsten and Bannach, Andreas and Davey, James and Ruppert, Tobias and Kohlhammer, J{\"o}rn},
  booktitle={Proc of IEEE VAST},
  pages={111--120},
  year={2011}
}
  %booktitle={Proc of IEEE Conference on Visual Analytics Science and Technology (VAST)},

@inproceedings{mcauley2013hidden,
  title={{Hidden factors and hidden topics: understanding rating dimensions with review text}},
  author={McAuley, Julian and Leskovec, Jure},
  booktitle={Proc of the 7th ACM conference on Recommender systems},
  pages={165--172},
  year={2013},
  organization={ACM}
}


@inproceedings{qu2010bag,
  title={{The bag-of-opinions method for review rating prediction from sparse text patterns}},
  author={Qu, Lizhen and Ifrim, Georgiana and Weikum, Gerhard},
  booktitle={Proc of COLING/ACL},
  pages={913--921},
  year={2010}
}



@article{rose2010automatic,
  title={Automatic keyword extraction from individual documents},
  author={Rose, Stuart and Engel, Dave and Cramer, Nick and Cowley, Wendy},
  journal={Text Mining},
  pages={1--20},
  year={2010}
}

@article{sinha2008incorporating,
  title={Incorporating domain knowledge into data mining classifiers: An application in indirect lending},
  author={Sinha, Atish P and Zhao, Huimin},
  journal={Decision Support Systems},
  volume={46},
  number={1},
  pages={287--299},
  year={2008},
  publisher={Elsevier}
}


@inproceedings{tang2008arnetminer,
  title={Arnetminer: extraction and mining of academic social networks},
  author={Tang, Jie and Zhang, Jing and Yao, Limin and Li, Juanzi and Zhang, Li and Su, Zhong},
  booktitle={Proc of ACM SIGKDD},
  pages={990--998},
  year={2008}
}

@article{tibshirani1996regression,
  title={Regression shrinkage and selection via the lasso},
  author={Tibshirani, Robert},
  journal={Journal of the Royal Statistical Society. Series B (Methodological)},
  pages={267--288},
  year={1996},
  publisher={JSTOR}
}

@inproceedings{zhang2006linear,
  title={Linear prediction models with graph regularization for web-page categorization},
  author={Zhang, Tong and Popescul, Alexandrin and Dom, Byron},
  booktitle={Proc of ACM SIGKDD},
  pages={821--826},
  year={2006}
}


@article{zhou2013tensor,
  title={Tensor regression with applications in neuroimaging data analysis},
  author={Zhou, Hua and Li, Lexin and Zhu, Hongtu},
  journal={Journal of the American Statistical Association},
  volume={108},
  number={502},
  pages={540--552},
  year={2013},
  publisher={Taylor \& Francis Group}
}

@article{zou2005regularization,
  title={Regularization and variable selection via the elastic net},
  author={Zou, Hui and Hastie, Trevor},
  journal={Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
  volume={67},
  number={2},
  pages={301--320},
  year={2005},
  publisher={Wiley Online Library}
}

@Article{auer2003using,
  title={Using confidence bounds for exploitation-exploration trade-offs},
  author={Auer, Peter},
  journal={Journal of Machine Learning Research},
  volume={3},
  pages={397--422},
  year={2003},
  publisher={JMLR. org}
}

@inproceedings{chu2011contextual,
author = {Chu, Wei and Lihong Li and Lev Reyzin and Robert E. Schapire},
title = {{Contextual bandits with linear payoff Functions}},
booktitle = {Proc of AISTATS},
year = {2011},
pages = {208--214},
}

@article{ruotsalo15interactive,
    author = {Tuukka Ruotsalo and Giulio Jacucci and Petri Myllym{\"a}ki and Samuel Kaski},
    journal = {CACM},
    language = {eng},
    number = {1},
    pages = {86-92},
    title = {{Interactive intent modeling: Information discovery beyond search}},
    volume = {58},
    year = {2015},
}

@inproceedings{Abbasi-Yadkori11improved,
 author = {Abbasi-Yadkori, Yasin and P\'{a}l, D\'{a}vid and Szepesv\'{a}ri, Csaba},
 title = {{Improved Algorithms for Linear Stochastic Bandits}},
 booktitle = {Proc of NIPS},
 series = {NIPS'11},
 year = {2011},
 isbn = {978-1-61839-599-3},
 location = {Granada, Spain},
 pages = {2312--2320},
 numpages = {9},
 url = {http://dl.acm.org/citation.cfm?id=2986459.2986717},
 acmid = {2986717},
 publisher = {Curran Associates Inc.},
 address = {USA},
} 

@inproceedings{ribeiro2016why,
  author    = {Marco T{\'{u}}lio Ribeiro and
               Sameer Singh and
               Carlos Guestrin},
  title     = {{"Why should {I} trust you?": Explaining the predictions of any classifier}},
  booktitle   =  {Proc of ACM SIGKDD},
  year      = {2016}
}

@article{Cano11a, 
    author={A. Cano and A. R. Masegosa and S. Moral}, 
    journal={IEEE Transactions on Systems, Man, and Cybernetics, Part B (Cybernetics)}, 
    title={{A Method for integrating expert knowledge when learning Bayesian networks from data}}, 
    year={2011}, 
    volume={41}, 
    number={5}, 
    pages={1382-1394}, 
    doi={10.1109/TSMCB.2011.2148197}, 
    ISSN={1083-4419}
}

@article{garthwaite13prior,
author = { Paul   H.   Garthwaite  and  Shafeeqah   A.   Al-Awadhi  and  Fadlalla   G.   Elfadaly  and  David   J.   Jenkinson },
title = {Prior distribution elicitation for generalized linear and piecewise-linear models},
journal = {Journal of Applied Statistics},
volume = {40},
number = {1},
pages = {59-75},
year = {2013},
doi = {10.1080/02664763.2012.734794},
}

@inproceedings{must-link-cannot-link,
  author = {Lu, Zhengdong and  Leen, Todd K.},
  title = {{Semi-supervised clustering with pairwise constraints: A discriminative approach}},
  booktitle = {Proc of AISTATS},
  pages = {299-306},
  year = 2007
}


@article{House2015bayesian,
  title={Bayesian Visual Analytics: {BaVa}},
  author={House, Leanna and Scotland, Leman and Han, Chao},
  journal={Statistical Analysis and Data Mining},
  volume={8},
  number={1},
  pages={1--13},
  year={2015},
  publisher={Wiley Online Library}
}

 @article{OLeary09,
  title = {Comparison of three expert elicitation methods for logistic regression on predicting the presence of the threatened brush-tailed rock-wallaby},
  author = {Rebecca A. O'Leary and Samantha Low Choy and Justine V. Murray and Mary Kynn and Robert Denham and Tara G. Martin and Kerrie Mengersen},
  journal = {Environmetrics},
  pages = {379--398},
  volume = 20,
  year = 2009
  }
  
@inproceedings{glowacka013directing,
 author = {Glowacka, Dorota and Ruotsalo, Tuukka and Konuyshkova, Ksenia and Athukorala, Kumaripaba and Kaski, Samuel and Jacucci, Giulio},
 title = {{Directing exploratory search: reinforcement learning from user interactions with keywords}},
 booktitle = {Proc of IUI},
 year = {2013},
 isbn = {978-1-4503-1965-2},
 location = {Santa Monica, California, USA},
 pages = {117--128},
 numpages = {12},
 url = {http://doi.acm.org/10.1145/2449396.2449413},
 doi = {10.1145/2449396.2449413},
 acmid = {2449413},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {adaptive interfaces, data mining, information filtering, machine learning, recommender systems},
}

@article{jones72astatistical,
    author = {Karen Spärck Jones},
    title = {A statistical interpretation of term specificity and its application in retrieval},
    journal = {Journal of Documentation},
    year = {1972},
    volume = {28},
    pages = {11--21}
}

@article{carpenter16stan,
    author = {Carpenter, Bob and Gelman, Andrew and Hoffman, Matt and Lee, Daniel and Goodrich, Ben and Betancourt, Michael and Brubaker, Michael A. and Guo, Jiqiang and Li, Peter and Riddell, Allen},
    year = {2016 (in press)},
    title = {Stan: A probabilistic programming language},
    journal = {Journal of Statistical Software},
    volume= {}
}

@inproceedings{soare16regression,
  title={{Regression with $n\to1$ by expert knowledge elicitation}},
  author={Soare, Marta and {Ammad-ud-din}, Muhammad and Kaski, Samuel},
  booktitle={Proc of ICMLA (to appear). arXiv preprint arXiv:1605.06477},
  year={2016}
}

@article{jones14prior,
author = {Geoffrey Jones and Wesley O. Johnson},
title = {{Prior elicitation: Interactive spreadsheet graphics with sliders can be fun, and informative}},
journal = {The American Statistician},
volume = {68},
number = {1},
pages = {42-51},
year = {2014},
}





% ADDED BY PEKKA ON OCT 12
@article{tian2014simple,
  title={A simple method for estimating interactions between a treatment and a large number of covariates},
  author={Tian, Lu and Alizadeh, Ash A and Gentles, Andrew J and Tibshirani, Robert},
  journal={Journal of the American Statistical Association},
  volume={109},
  number={508},
  pages={1517--1532},
  year={2014},
  publisher={Taylor \& Francis}
}

% ADDED BY PEKKA ON OCT 12
@article{papillon2013comparison,
  title={Comparison and validation of genomic predictors for anticancer drug sensitivity},
  author={Papillon-Cavanagh, Simon and De Jay, Nicolas and Hachem, Nehme and Olsen, Catharina and Bontempi, Gianluca and Aerts, Hugo JWL and Quackenbush, John and Haibe-Kains, Benjamin},
  journal={Journal of the American Medical Informatics Association},
  volume={20},
  number={4},
  pages={597--602},
  year={2013},
  publisher={The Oxford University Press}
}

% ADDED BY PEKKA ON OCT 12
@inproceedings{wang2011sparse,
  title={Sparse multi-task regression and feature selection to identify brain imaging predictors for memory performance},
  author={Wang, Hua and Nie, Feiping and Huang, Heng and Risacher, Shannon and Ding, Chris and Saykin, Andrew J and Shen, Li and others},
  booktitle={Proc of ICCV},
  pages={557--562},
  year={2011}
}

% ADDED BY IIRIS ON OCT 12
@article{kadane80interactive,
author = { Joseph B.   Kadane  and  James M.   Dickey  and  Robert L.   Winkler  and  Wayne S.   Smith  and  Stephen C.   Peters },
title = {{Interactive elicitation of opinion for a normal linear model}},
journal = {Journal of the American Statistical Association},
volume = {75},
number = {372},
pages = {845-854},
year = {1980},
}

==> supp_predictionmodel.tex <==
%\subsubsection*{Prediction Model}
As input, the prediction model takes training data points $(\mathbf{x}_{i},y_{i}),~i=1,\ldots,N,$ where $\mathbf{x}_{i}\in\mathbb{R}^{K}$ and $y_{i}\in\mathbb{R}$, and a vector of relevances $\mathbf{r}\in\{0,1\}^{K},$where $r_{j}=1,$ if the feature is relevant, i.e., has received positive feedback. Otherwise, $r_{j}=0$.

\begin{figure}[b]
    \centering
    \includegraphics[width=\textwidth]{prior_fig.png}
    \caption{Prior distributions of the parameters of the prediction model}
    \label{fig:priors}
\end{figure}

We assume the target $y_{i}$ depends linearly on the predictor $\mathbf{x}_{i}$%
\[
y_{i}\sim N(\mathbf{x}_{i}^{T}\mathbf{w},\sigma^{2}),\text{ }i=1\ldots,N,
\]
where $\mathbf{w\in}\mathbb{R}^{K}$ is a vector of regression coefficients and $\sigma^{2}$ is the variance of the Gaussian noise. The relevances of the predictors $\mathbf{r}$ affect the prior distributions of the elements of $\mathbf{w}$ as follows%
\begin{align*}
w_{j}  & \sim N(0,\sigma_{0}^{2}),\text{ if }r_{j}=0,\\
w_{j}  & \sim\text{half-}N(0,a\sigma_{0}^{2}),\text{ if }r_{j}=1.
\end{align*}
Here, half-$N$ denotes the half-normal distribution. The intuition is that if a feature is relevant, the corresponding regression weight is assumed to have a prior distribution constrained to be positive (see, Fig. \ref{fig:priors}A). The multiplier $a$ determines the ratio of the variance parameters between relevant and non-relevant features, and is given a prior distribution
\[
a\sim1+\text{half-}N(0,12.5\pi).
\]
This constrains $a$ to be greater than $1$ and have mean 6, according to a weakly informative prior (see Fig. \ref{fig:priors}B). This corresponds to the expectation that regression coefficients of the relevant features are greater in magnitude than the coefficients of the non-relevant features.

The term $\sigma_{0}^{2}$ appearing in the prior variances of the regression
coefficients of both relevant and non-relevant features is specified by
investigating the variance of the linear predictions. A direct integration of
regression weights $\mathbf{w}$, conditional on parameters $a$ and $\sigma
_{0}^{2}$, gives%
\begin{align}
E_{\mathbf{w}}\left[  Var(\mathbf{x}^{T}\mathbf{w)}\right]   &  =\frac{1}{N}%
%TCIMACRO{\tsum \nolimits_{i}}%
%BeginExpansion
{\textstyle\sum\nolimits_{i}}
%EndExpansion
\mathbf{x}_{i}^{T}E_{\mathbf{w}}\left[  \mathbf{ww}^{T}\right]  \mathbf{x}%
_{i}\nonumber\\
&  =\sigma_{0}^{2}(n_{-}+an_{+})+\frac{2a\sigma_{0}^{2}}{\pi}\sum_{k\in R}%
\sum_{\substack{h\in R\\h\neq k}}\sigma_{kh}\label{two_terms}\\%
&  \approx\sigma_{0}^{2}(n_{-}+an_{+}),\label{approximation}%
\end{align}
where $n_{+}$ and $n_{-}$ are the numbers of relevant and non-relevant
features, $R$ is the set of all relevant features, and $\sigma_{kh}$ is the
covariance between the $k^{th}$ and $h^{th}$ features. In practice the second
term in Equation \ref{two_terms} is less than 25\% of the first term, and
therefore, we retain only the first term to keep the computations simple (this
is exact when the relevant features are uncorrelated). Let
$\xi$ denote the proportion of variance explained by the prediction model.
Assuming $y$ is normalized, the proportion of variance explained is given by Equation \ref{approximation}, and we can solve for $\sigma_{0}^{2}$ for any $\xi$ by
using:%
\[
\sigma_{0}^{2}(n_{-}+an_{+})=\xi,
\]
which yields%
\begin{equation}
\sigma_{0}^{2}=\frac{\xi}{n_{-}+an_{+}}.\label{sigma_0}%
\end{equation}
We define a prior for $\xi$ as
\[
\xi\sim Beta(1,9),
\]
shown in Fig. \ref{fig:priors}C, which corresponds to the expectation that
approximately 10\% of the variance of the target is explained by the
prediction model. This further imposes a prior on $\sigma_{0}^{2}$ through
Equation \ref{sigma_0}. Finally, we place the following prior on noise
variance%
\[
\sigma\sim\text{half-}N(0,1),
\]
which completes the definition of the prediction model. The model is implemented using the probabilistic programming language Stan \cite{carpenter16stan}.

